A Concurrent Perspective on Smart Contracts

In this paper, we explore remarkable similarities between multi-transactional behaviors of smart contracts in cryptocurrencies such as Ethereum and classical problems of shared-memory concurrency. We examine two real-world examples from the Ethereum blockchain and analyzing how they are vulnerable to bugs that are closely reminiscent to those that often occur in traditional concurrent programs. We then elaborate on the relation between observable contract behaviors and well-studied concurrency topics, such as atomicity, interference, synchronization, and resource ownership. The described contracts-as-concurrent-objects analogy provides deeper understanding of potential threats for smart contracts, indicate better engineering practices, and enable applications of existing state-of-the-art formal verification techniques.

==> compos.tex <==
\section{Composing the Contracts}
\label{sec:comp-atom-contr}

A synchronization discipline, such as the one provided by an exclusive
ownership or a read/write lock should not be an inherent part of a
contract. 

\begin{enumerate}

\item Lock should be an external servise
\item Contract composition
\item Real-world examples

\end{enumerate}

\is{Say why do we want to have a lock as an external service}

\todo{Mention linearizability}

